Near-Optimal Provable Uniform Convergence in Offline Policy Evaluation for Reinforcement Learning

The problem of Offline Policy Evaluation (OPE) in Reinforcement Learning (RL) is a critical step towards applying RL in real-life applications. Existing work on OPE mostly focus on evaluating a fixed target policy $\pi$, which does not provide useful bounds for offline policy learning as $\pi$ will then be data-dependent. We address this problem by simultaneously evaluating all policies in a policy class $\Pi$ -- uniform convergence in OPE -- and obtain nearly optimal error bounds for a number of global / local policy classes. Our results imply that the model-based planning achieves an optimal episode complexity of $\widetilde{O}(H^3/d_m\epsilon^2)$ in identifying an $\epsilon$-optimal policy under the time-inhomogeneous episodic MDP model ($H$ is the planning horizon, $d_m$ is a quantity that reflects the exploration of the logging policy $\mu$). To the best of our knowledge, this is the first time the optimal rate is shown to be possible for the offline RL setting and the paper is the first that systematically investigates the uniform convergence in OPE.

==> sections/method.tex <==

% !TEX root = ../Uniform_OPE_icml.tex

\subsection{Tabular Marginalized Importance Sampling Estimator}

\textbf{We stick with the tabular marginalized importance sampling estimator (TMIS). }

In addition to the non-stationary, finite horizon tabular MDP $M=(\mathcal{S},\mathcal{A},r,T,d_1,H)$ (where $S:=|\mathcal{S}|<\infty$ and $A:=|\mathcal{A}|<\infty$), non-stationary logging policy $\mu$ and target policy $\pi$ in Section~\ref{sec:preliminary}, we denote $d^\mu_t(s_t,a_t)$ and $d^\pi_t(s_t,a_t)$ the induced joint state-action distribution at time $t$ and the state distribution counterparts $d^\mu_t(s_t)$ and $d^\pi_t(s_t)$, satisfying $d^{\pi}_t(s_t,a_t)=d^{\pi}_t(s_t)\cdot \pi(a_t|s_t)$.\footnote{For $\mu$, $d^{\mu}_t(s_t,a_t)=d^{\mu}_t(s_t)\cdot \mu(a_t|s_t)$.} The initial distributions are identical $d_1^\mu=d^\pi_1=d_1$. Moreover, we use $P^\pi_{i,j}\in\mathbb{R}^{S\times S}, \;\forall j<i$ to represent the state transition probability from step $j$ to step $i$ under policy $\pi$, where $P^\pi_{t+1,t}(s^\prime|s)=\sum_a P_{t+1,t}(s^\prime|s,a)\pi_t(a|s)$.  The marginal state distribution vector ${d}_t^\pi(\cdot)$ satisfies
${d}_t^\pi  = {P}^{\pi}_{t,t-1} {d}_{t-1}^\pi,$

Historical data $\mathcal{D}=\left\lbrace (s_t^{(i)},a_t^{(i)},r_t^{(i)})\right\rbrace_{i\in[n]}^{t\in[H]} $ was obtained by logging policy $\mu$ and we can only use $\mathcal{D}$ to estimate the value of target policy $\pi$, \emph{i.e.} $v^\pi$. Suppose we only assume knowledge about $\pi(a|s)$ for all $(s,a)\in\mathcal{S}\times\mathcal{A}$ and \emph{do not observe} $r_t(s_t,a_t)$ for any actions other than the noisy immediate reward $r_t^{(i)}$ after observing $s_t^{(i)},a_t^{(i)}$. 

\begin{assumption}[Bounded rewards]\label{assume1}
	 $\forall \;t=1,...,H$ and $i=1,...,n$, $0\leq r^{(i)}_t\leq R_{\max}$.
\end{assumption}
The bounded reward assumption can be relaxed to:  $\exists R_{\max},\sigma<+\infty$ such that $0\leq \mathbb{E}[r_t|s_t,a_t,s_{t+1}]\leq R_{\max}$, $\mathrm{Var}[r_t|s_t,a_t,s_{t+1}]\leq \sigma^2$ (as in \citet{xie2019towards}), for achieving Cramer-Rao lower bound. However, the boundedness will become essential for applying concentrate inequalities in deriving high probability bounds.

\begin{assumption}\label{assume2}
	Logging policy $\mu$ obeys $d_m:=\min_{t,s_t}d^\mu_t(s_t)>0$.
\end{assumption}
This assumption is always required for the consistency of off-policy evaluation estimator. 

\begin{assumption}[Bounded weights]\label{assume3}
	$\tau_s:=\max_{t,s_t}\frac{d^\pi_t(s_t)}{d^\mu_t(s_t)}<+\infty$ and $\tau_a:=\max_{t,s_t,a_t}\frac{\pi(a_t|s_t)}{\mu(a_t|s_t)}<+\infty$.
\end{assumption}
Assumption~\ref{assume3} is also necessary for discrete state and actions, as otherwise the second moments of the importance weight would be unbounded and the MSE of estimators will become intractable . The bound on $\tau_s$ is natural since $\tau_s\leq \max_{t,s_t}\frac{1}{d^\mu_t(s_t)}=\frac{1}{\min_{t,s_t}d^\mu_t(s_t)}=\frac{1}{d_m}$ and it's finite by the Assumption~\ref{assume2}; similarly, $\tau_a<\infty$ is also automatically satisfied if $\min_{t,s_t,a_t}\mu(a_t|s_t)>0$.  

\subsection{Tabular-MIS estimator}

Marginalized importance sampling directly estimates
the marginalized state visitation distribution $\widehat{d}_t$ and defines the MIS estimator:

\begin{equation}\label{MIS_def}
\widehat{v}^\pi_{MIS} =\frac{1}{n}\sum_{i=1}^n\sum_{t=1}^H\frac{\widehat{d}^\pi_t(s_t^{(i)})}{\widehat{d}^\mu_t(s^{(i)}_t)}\widehat{r}^\pi_t(s^{(i)}).
\end{equation}
and $\widehat{d}^\mu_t(\cdot)$ is directly estimated using the empirical mean, \emph{i.e.} $\widehat{d}^\mu_t(s_t):=\frac{1}{n}\sum_i \mathbf{1}(s_t^{(i)}=s_t):=\frac{n_{s_t}}{n}$ whenever $n_{s_t}>0$ and $\widehat{d}^\pi_t(s_t)/\widehat{d}^\mu_t(s_t)=0$ when $n_{s_t}=0$. Then the MIS estimator \eqref{MIS_def} becomes:
\begin{equation}\label{MIS}
\widehat{v}^\pi_{MIS}=\sum_{t=1}^H\sum_{s_t}\widehat{d}^\pi_t(s_t)\widehat{r}^\pi_t(s_t)
\end{equation}

\paragraph{Construction of \TMIS .} 
  
We can construct empirical estimates for $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ as: 
{\small
\begin{equation}\label{eq:tabular_MIS_construction}
%\hspace{-3.5mm}
\begin{aligned}
\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})&=\frac{\sum_{i=1}^n\mathbf{1}[(s^{(i)}_{t+1},a^{(i)}_t,s^{(i)}_t)=(s_{t+1},s_{t},a_{t})]}{n_{s_{t},a_{t}}}\\
\widehat{r}_t(s_t,a_t)&=\frac{\sum_{i=1}^n r_t^{(i)}\mathbf{1}[(s^{(i)}_t,a^{(i)}_t)=(s_t,a_t)]}{n_{s_t,a_t}},\\
\end{aligned}
\end{equation}
}
where we set $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})=0$ and $\widehat{r}_t(s_t,a_t)=0$ if $n_{s_t,a_t}=0$, with $n_{s_t,a_t}$ the empirical visitation frequency to state-action $(s_t,a_t)$ at time $t$. The corresponding estimation of $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ are defined as:

\begin{equation}\label{eq:tabular_MIS_construction2}
\begin{aligned}
\widehat{P}^\pi_t(s_t|&s_{t-1})=\sum_{a_{t-1}}\widehat{P}_t(s_t|s_{t-1},a_{t-1})\pi(a_{t-1}|s_{t-1}),\\
\widehat{r}^\pi_t(s_t)&=\sum_{a_t}\widehat{r}_t(s_t,a_t)\pi(a_t|s_t),\;\widehat{d}^\pi_t=\widehat{P}^\pi_t\widehat{d}^\pi_{t-1}. 
\end{aligned}
\end{equation}




%\red{However, model-based approaches are not well-understood even in tabular setting.  Some discussions and summary of the understanding of tabular methods are here: \url{http://nanjiang.cs.illinois.edu/files/cs598/note3.pdf}
%In particular, check the "Simulation Lemma", and check out the various ``naive approaches'' to analyze the model-based methods.}


